Causal SAR ATR with Limited Data via Dual Invariance

Synthetic aperture radar automatic target recognition (SAR ATR) with limited data has recently been a hot research topic to enhance weak generalization. Despite many excellent methods being proposed, a fundamental theory is lacked to explain what problem the limited SAR data causes, leading to weak generalization of ATR. In this paper, we establish a causal ATR model demonstrating that noise $N$ that could be blocked with ample SAR data, becomes a confounder with limited data for recognition. As a result, it has a detrimental causal effect damaging the efficacy of feature $X$ extracted from SAR images, leading to weak generalization of SAR ATR with limited data. The effect of $N$ on feature can be estimated and eliminated by using backdoor adjustment to pursue the direct causality between $X$ and the predicted class $Y$. However, it is difficult for SAR images to precisely estimate and eliminated the effect of $N$ on $X$. The limited SAR data scarcely powers the majority of existing optimization losses based on empirical risk minimization (ERM), thus making it difficult to effectively eliminate $N$'s effect. To tackle with difficult estimation and elimination of $N$'s effect, we propose a dual invariance comprising the inner-class invariant proxy and the noise-invariance loss. Motivated by tackling change with invariance, the inner-class invariant proxy facilitates precise estimation of $N$'s effect on $X$ by obtaining accurate invariant features for each class with the limited data. The noise-invariance loss transitions the ERM's data quantity necessity into a need for noise environment annotations, effectively eliminating $N$'s effect on $X$ by cleverly applying the previous $N$'s estimation as the noise environment annotations. Experiments on three benchmark datasets indicate that the proposed method achieves superior performance.

==> not_used/name.tex <==
\section{Related Works}
\label{2}

\subsection{SAR ATR with Limited Data} 

\subsection{Causal Inference}
Causal inference is a fundamental problem in machine learning and has been the subject of extensive research in recent years. Many existing works in causal inference can be broadly categorized into two categories: causal discovery and causal effect estimation.

Causal discovery aims to infer the causal structure of a system from observational data. A popular approach in causal discovery is to use graphical models, such as Bayesian networks [14] and causal Bayesian networks [15], to represent the causal relationships between variables. Other methods include constraint-based algorithms [16] and information-theoretic methods [17].

Causal effect estimation, on the other hand, aims to estimate the causal effect of a treatment on an outcome. This is often done using randomized controlled trials (RCTs), where the treatment is randomly assigned to the subjects. However, in many cases, RCTs are not feasible or ethical, and we need to rely on observational data. In this case, we can use methods such as propensity score matching [18] and inverse probability weighting [19] to estimate the causal effect.

Recently, there has been a growing interest in developing methods for causal inference in the presence of confounders, where the treatment and outcome are affected by common causes. These methods aim to control for confounding variables by either adjusting for them in the analysis or by using experimental designs that minimize their impact [20]. One popular approach is the use of instrumental variables, which are variables that affect the treatment but not the outcome, to estimate the causal effect [21].

In addition to these methods, there has been increasing interest in the use of deep learning for causal inference. Deep learning models can be used to estimate causal effects from observational data by learning the functional form of the causal relationship between variables [22]. Some recent works have also explored the use of deep learning for causal discovery [23,24]. However, the use of deep learning for causal inference is still in its early stages, and more research is needed to fully explore its potential.
